On the connection between Noise-Contrastive Estimation and Contrastive Divergence

Noise-contrastive estimation (NCE) is a popular method for estimating unnormalised probabilistic models, such as energy-based models, which are effective for modelling complex data distributions. Unlike classical maximum likelihood (ML) estimation that relies on importance sampling (resulting in ML-IS) or MCMC (resulting in contrastive divergence, CD), NCE uses a proxy criterion to avoid the need for evaluating an often intractable normalisation constant. Despite apparent conceptual differences, we show that two NCE criteria, ranking NCE (RNCE) and conditional NCE (CNCE), can be viewed as ML estimation methods. Specifically, RNCE is equivalent to ML estimation combined with conditional importance sampling, and both RNCE and CNCE are special cases of CD. These findings bridge the gap between the two method classes and allow us to apply techniques from the ML-IS and CD literature to NCE, offering several advantageous extensions.

==> content/app/cis_perspective.tex <==
\subsubsection{NCE from CIS}
%
(Note that in constrast to the IS estimator, we here include $\y_0 = \y$ in the sum).
Here, we Gibbs sample from the joint pdf

Let 
\begin{align}
    \numNeg' &\sim \categorical{\frac{1}{\NumNeg + 1}} \nonumber \\
    \y_\numNeg' &\sim \pModel(\y) \nonumber \\ 
    \y_\numNeg &\sim \pNoise(\y),\, \numNeg \neq \numNeg', \numNeg = 0, \dots, \NumNeg\\
    \y_{-\numNeg'} &\eqDef (\y_0, \dots, \y_{\numNeg'-1}, \y_{\numNeg'+1}, \dots, \y_\NumNeg)
\end{align}
Then we can write the joint distribution (and its factorisations)
\begin{align}
  \label{eq:cis:joint_pdf}
  \pp_{\param}(\numNeg', \yNegSeq{0})
  &= \overbrace{\frac{1}{\NumNeg + 1 }}^{\pp(\numNeg')}
  \times \overbrace{\pModel(\y_{\numNeg'})}^{\pp(\y_{\numNeg'} \vert \numNeg')}
  \times \overbrace{ \prod_{\numNeg \neq \numNeg'} \pNoise(\y_{\numNeg}) }^{ \pp(\ySeqNot{\numNeg'}) } \nonumber \\
  %
  &= \frac{1}{(\NumNeg + 1) \partFn} \w(\y_{\numNeg'}) \prod_{\numNeg = 0}^{\NumNeg} \pNoise(\y_\numNeg) \nonumber \\
  %
  &= \overbrace{ \frac{\w(\y_{\numNeg'})}{\sum_{\numNeg''=0}^{\NumNeg} \w(\y_{\numNeg''})} }^{\pp(\numNeg' \vert \yNegSeq{0})}
  \times \overbrace{ \frac{\partFnHatCis}{\partFn} \prod_{\numNeg = 0}^{\NumNeg} \pNoise(\y_{\numNeg}) }^{ \pp(\yNegSeq{0}) },
\end{align}

==> content/app/cond_nce_gibbs.tex <==
To formulate this as a Gibbs sampler, start with
%
\begin{align}
    &\bernoullivar \sim \bernoulli \left(\frac{1}{2}\right), \nonumber \\
    &\y, \y' \vert \bernoullivar = 1 \sim \pModel(\y)\pNoise(\y' \vert \y) \nonumber \\
    &\y, \y' \vert \bernoullivar = 0 \sim \pModel(\y')\pNoise(\y \vert \y').
\end{align}
%
Then,
\begin{align}
    \pp(\bernoullivar, \y, \y') &= \overbrace{\frac{1}{2}}^{\pp(\bernoullivar)} \times \overbrace{( \bernoullivar\pModel(\y)\pNoise(\y' \vert \y) + (1-\bernoullivar)\pModel(\y')\pNoise(\y \vert \y')}^{\pp(\y, \y'\mid \bernoullivar))} \nonumber \\
    &=  \overbrace{\frac{\bernoullivar\pModel(\y)\pNoise(\y' \vert \y) + (1-\bernoullivar)\pModel(\y')\pNoise(\y \vert \y')}{\pModel(\y)\pNoise(\y' \vert \y) + \pModel(\y')\pNoise(\y \vert \y')}}^{\pp(\bernoullivar \vert \y, \y')}  \times \overbrace{\frac{1}{2}(\pModel(\y)\pNoise(\y' \vert \y) + \pModel(\y')\pNoise(\y \vert \y'))}^{\pp(\y, \y')},
\end{align}
from which we can Gibbs sample
\begin{align}
    &\bernoullivar \vert \y, \y' \sim \pp(\bernoullivar \vert \y, \y'), \nonumber \\
    & \y, \y' \mid \bernoullivar \sim \pp(\y, \y' \vert \bernoullivar).
\end{align}

==> content/app/cond_nce_mh.tex <==
\subsection{Validity of CNCE MCMC kernel}
\label{app:detailed_bal}
We show that the kernel defined for the CNCE criterion fulfils detailed balance, and therefore that it is $\pModel(\y)$-invariant. The detailed balance condition follows as [Ref]
\begin{align}
    \pModel(\y_0)\kernel(\y_1\vert \y_0) = \pModel(\y_1)\kernel(\y_0\vert \y_1).
\end{align}
%
The detailed balance condition is trivially satisfied for $\y'=\y$. For the other case, $\y_1 \neq \y_0$, we can rewrite the kernel as
%
\begin{align}
    \kernel(\y_1\vert \y_0) = \pp(\bernoullivar=1 \vert \y_0, \y_1) \pNoise(\y_1\vert \y_0).
\end{align}
%
In this case, we have
\begin{align}
    \pModel(\y_0)\kernel(\y_1\vert \y_0) &= \pModel(\y_0) \pp(\bernoullivar=1 \vert \y_0, \y_1) \pNoise(\y_1\vert \y_0) \nonumber \\
    &=  \pModel(\y_0) \frac{\pModel(\y_1) \pNoise(\y_0 \vert \y_1)}{\pModel(\y_1) \pNoise(\y_0 \vert \y_1) + \pModel(\y_0) \pNoise(\y_1 \vert \y_0)} \pNoise(\y_1\vert \y_0)
     \nonumber \\
    &=  \pModel(\y_1) \frac{\pModel(\y_0) \pNoise(\y_1 \vert \y_0)}{\pModel(\y_1) \pNoise(\y_0 \vert \y_1) + \pModel(\y_0) \pNoise(\y_1 \vert \y_0)} \pNoise(\y_0 \vert \y_1) \nonumber \\
    &= \pModel(\y_1) \pp(\bernoullivar=0 \vert \y_0, \y_1) \pNoise(\y_0 \vert \y_1)
    \nonumber \\
    &= \pModel(\y_1) \kernel(\y_0 \vert \y_1),
\end{align}
which shows that the detailed balance condition is fulfilled.

==> content/app/cond_nce_multiple_steps_derivation.tex <==
\subsection{Conditional NCE with multiple steps}

For the conditional NCE criterion with multiple MCMC steps, we use the conditional sampling scheme as the one used to derive the conditional NCE criterion. We take $\totMcmcSteps$ MCMC steps, where we at each step $\mcmcStep$ sample an indicator variable $\bernoullivar^{(\mcmcStep)} \in \{0, 1\}$ and use $\y^{(\mcmcStep + 1)} = \y_{\bernoullivar}^{(\mcmcStep)}$ if $\bernoullivar^{(\mcmcStep)} = 1$ and $\y^{(\mcmcStep + 1)} = \y_1^{(\mcmcStep)}$ otherwise. Marginalising over all indicator variables, the second term in the gradient is estimated as
%
\begin{align}
    &\expect[\kernel(\y' \vert \y)]{ \log \pUnnorm(\y') } \nonumber \\
    &= \expect[\pp(\y_1^{(1)} \vert \y_0^{(1)})]{ \expect[\pp(\bernoullivar^{(1)} \vert \y_{0:1}^{(1)})]{ \ldots \expect[\pp(\y_1^{(\totMcmcSteps - 1)} \vert \y_0^{(\totMcmcSteps - 1)})]{ \expect[\pp(\bernoullivar^{(\totMcmcSteps - 1)} \vert  \y_{0:1}^{(\totMcmcSteps - 1)})]    {   \expect[\pp(\y_1^{(\totMcmcSteps)} \vert \y_0^{(\totMcmcSteps)})]{ \expect[\pp(\bernoullivar^{(\totMcmcSteps)} \vert \y_{0:1}^{(\totMcmcSteps)})] {  \log \pUnnorm(\y_{\bernoullivar})}}  }} \ldots }} 
\end{align}



==> content/app/nce_ranking_crit_grad_ebm.tex <==
For EBMs, with
\begin{align*}
    \log \pUnnorm(\y) = - \energy(\y),
\end{align*}
The NCE ranking criterion follows as
\begin{align}
  \label{eq:nce:rank_crit:neg_log}
  - \log \p(\numNeg = 0 \vert \y_0, \y_1, \dots \y_{\NumNeg}) &=- \log \frac{ \exp(-\energy(\y_0) - \log \pNoise(\y_{0})) }{ \sum_{\numNeg=0}^{\NumNeg} \exp(-\energy(\y_{\numNeg}) - \log \pNoise(\y_{\numNeg})) },
\end{align}
with gradient
\begin{align}
  \label{eq:nce:rank_crit:grad}
  &- \gradP{ \log \p(\numNeg = 0 \vert \y_0, \y_1, \dots \y_{\NumNeg}) } 
  = \gradP{ \energy(\y_0) } - \sum_{\numNeg=0}^{\NumNeg} \wNorm{0}(\y_{\numNeg}) \gradP{\energy(\y_{\numNeg})}.
\end{align}

==> content/app/nce_ranking_multiple_steps_derivation.tex <==
\subsubsection{NCE ranking with multiple steps}

Assume we estimate the second term in \cref{eq:cd:grad} using the same conditional sampling scheme as the one used to derive the NCE ranking criterion but taking $\totMcmcSteps$ MCMC steps instead of just one. At each step $\mcmcStep$ we sample an index $\selectInd^{(\mcmcStep)} \in {0, \ldots, \NumNeg}$ and use $\y_0^{(\mcmcStep + 1)} = \y_{\selectInd^{(\mcmcStep)}}^{(\mcmcStep)}$. Then, the estimate follows as 
%
\begin{align}
    &\expect[\kernel(\y' \vert \y)]{ \log \pUnnorm(\y') } \nonumber \\
    &= \expect[\pp(\y_{1:\NumNeg}^{(1)} \vert \y_0^{(1)})]{ \expect[\pp(\selectInd^{(1)} \vert \y_{0:\NumNeg}^{(1)})]{ \ldots \expect[\pp(\y_{1:\NumNeg}^{(\totMcmcSteps - 1)} \vert \y_0^{(\totMcmcSteps - 1)})]{ \expect[\pp(\selectInd^{(\totMcmcSteps - 1)} \vert \y_{0:\NumNeg}^{(\totMcmcSteps - 1)})]    {   \expect[\pp(\y_{1:\NumNeg}^{(\totMcmcSteps)} \vert \y_0^{(\totMcmcSteps)})]{ \expect[\pp(\selectInd^{(\totMcmcSteps)} \vert \y_{0:\NumNeg}^{(\totMcmcSteps)})] {  \log \pUnnorm(\y_{\selectInd^{(\totMcmcSteps)}}) }}  }} \ldots }} 
\end{align}
%

==> content/experiments/pers_cnce.tex <==
%\subsection{Persistent CNCE}
We additionally investigate the performance improvement of applying persistence to CNCE (P-CNCE) as well as MH-CNCE (P-MH-CNCE) and add these to the ring model experiments. Results are reported in \cref{fig:acc_prob_exp}, including median acceptance probabilities of both P-CNCE and P-MH-CNCE, calculated when training with P-CNCE. 

%
The use of persistence does not only lead to faster converge but also improves both median and worst-case performance. The benefits of replacing the acceptance probability of CNCE is less evident when combined with persistence, although the median acceptance probability of P-MH-CNCE is overall larger than that of P-CNCE. 

==> content/extensions/cond_nce_multiple_steps.tex <==
\subsection{Conditional NCE with multiple MCMC steps}
Just as for the NCE ranking criterion, we introduce conditional NCE with $\totMcmcSteps$ MCMC steps, this time using the kernel outlined for the conditional NCE criterion given in \cref{alg:cd_cnce:cnce_kernel}. Similar to the preceding algorithm, we condition on the previous sample, i.e. $\y_0^{(\mcmcStep)} = \y_{\bernoullivar}^{(\mcmcStep - 1)}$, at each step. Marginalising over the indicator variables, $\bernoullivar$, the second term in \cref{eq:cd:grad} is estimated according to
%
\begin{align}
\label{eq:cd_cnce_multi_steps:grad}
    &\expect[\condKernel(\y' \vert \y_0)]{ \gradP{\log \pUnnorm(\y')} } \approx \frac{1}{\totMcmcSteps} \sum_{\mcmcStep = 1}^{\totMcmcSteps} \wNorm{}(\y_0^{(\mcmcStep)} \mid \y_{\numNeg}^{(\mcmcStep)}) \gradP{\log \pUnnorm(\y_0^{(\mcmcStep)})} \nonumber \\ 
    &\quad + \wNorm{} (\y_{\numNeg}^{(\mcmcStep)} \mid \y_0^{(\mcmcStep)}) \gradP{\log \pUnnorm(\y_{\numNeg}^{(\mcmcStep)})}.
\end{align}
Just as for \cref{eq:cd_rnce_multi_steps:grad}, the final gradient estimate is taken as an average over the individual estimates obtained at each MCMC step.
